CRINN: Contrastive Reinforcement Learning for Approximate Nearest Neighbor Search

Approximate nearest-neighbor search (ANNS) algorithms have become increasingly critical for recent AI applications, particularly in retrieval-augmented generation (RAG) and agent-based LLM applications. In this paper, we present CRINN, a new paradigm for ANNS algorithms. CRINN treats ANNS optimization as a reinforcement learning problem where execution speed serves as the reward signal. This approach enables the automatic generation of progressively faster ANNS implementations while maintaining accuracy constraints. Our experimental evaluation demonstrates CRINN's effectiveness across six widely-used NNS benchmark datasets. When compared against state-of-the-art open-source ANNS algorithms, CRINN achieves best performance on three of them (GIST-960-Euclidean, MNIST-784-Euclidean, and GloVe-25-angular), and tied for first place on two of them (SIFT-128-Euclidean and GloVe-25-angular). The implications of CRINN's success reach well beyond ANNS optimization: It validates that LLMs augmented with reinforcement learning can function as an effective tool for automating sophisticated algorithmic optimizations that demand specialized knowledge and labor-intensive manual refinement. Code can be found at https://github.com/ornith-ai/CRINN

==> header_style.tex <==
% 一次性加载 geometry，给出页边距和 \headheight
% 增加 headsep 来让第一页页眉和正文之间有更大间距
\usepackage[margin=3cm, headheight=50pt, headsep=0pt]{geometry}

\usepackage{graphicx}   % 插图
\usepackage{fancyhdr}   % 自定义页眉页脚

% ------- 页眉定义 -------
\pagestyle{fancy}       % 默认页眉样式
\fancyhf{}              % 清空

% 删除默认页面的横线
\renewcommand{\headrulewidth}{0pt}

\begin{comment}
% 左侧：logo + 项目名，可按需删掉 \textsc{}
\fancyhead[L]{%
  \raisebox{-0.25\height}{\includegraphics[height=20pt]{./header.png}}%
}

% 右侧放页码示例（可不要）
\fancyhead[R]{}

% (2) 横向"拉长"：把页眉区域往左右各伸出 2.5 cm
\fancyheadoffset[L]{0.2cm}
\fancyheadoffset[R]{0.2cm}
\end{comment}

% 让首页 (plain) 同样使用这种页眉
\fancypagestyle{plain}{%
  \fancyhf{}
  \fancyhead[L]{%
    % 方法1：通过添加 \vspace 来让页眉内容下移
    \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{\includegraphics[height=25pt]{./header.png}}%
      \vfill
    }%
  }
  \fancyhead[R]{
  \vbox to 25pt{%
      \vfill
      \raisebox{25pt}{}
      \vfill
    }%
  }
  \renewcommand{\headrulewidth}{0.7pt}  % 保留第一页的横线
  \fancyheadoffset[L]{0cm}
  \fancyheadoffset[R]{0cm}
}

% 如果只想让第一页的页眉和正文间距更大，可以在文档开始处使用：
% \thispagestyle{plain}
% \vspace{20pt}  % 在第一页正文开始前添加额外空间

==> images/training_recipe.tex <==

\begin{figure*}[h]
 \centering
 \begin{adjustbox}{margin=-0.5cm 0cm 0cm 0cm}
 \begin{minipage}[c]{\textwidth}
 \centering
\includegraphics[scale=0.12]{./images/pipeline_v3.jpg}
\caption{Overview of the CUDA-L1 training pipeline. The approach consists of three progressive stages:
\textbf{(1) Stage 1: Supervised Fine-tuning with Data Augmentation} -- We augment the training dataset with  CUDA code variants generated by LLMs and fine-tune the base model on executable and correct implementations to establish foundational CUDA knowledge.
\textbf{(2) Stage 2: Self-supervised Learning} -- The model iteratively generates CUDA kernels, validates their correctness and executability, and trains on successfully validated examples, enabling autonomous improvement without human supervision.
\textbf{(3) Stage 3: Contrastive Reinforcement Learning} -- We employ contrastive learning with execution-time rewards, training the model to distinguish between faster and slower CUDA implementations, ultimately optimizing for superior performance.}
\label{fig:pipeline_figure}
 \end{minipage}
 \end{adjustbox}
 \end{figure*}

==> tables/conv3d.tex <==
\begin{table*}
 \centering
 \begin{adjustbox}{margin=-0.2cm 0cm 0cm 0cm}
 \begin{minipage}[c]{\textwidth}
 \centering
\includegraphics[scale=0.4]{./tables/conv3d}
\caption{Speedup achieved by different CUDA optimization techniques on the Conv3d task.}
\label{fig:conv3d}
 \end{minipage}
 \end{adjustbox}
 \end{table*}
